LDA2Net: Digging under the surface of COVID-19 topics in scientific literature

During the COVID-19 pandemic, the scientific literature related to SARS-COV-2 has been growing dramatically, both in terms of the number of publications and of its impact on people's life. This literature encompasses a varied set of sensible topics, ranging from vaccination, to protective equipment efficacy, to lockdown policy evaluation. Up to now, hundreds of thousands of papers have been uploaded on online repositories and published in scientific journals. As a result, the development of digital methods that allow an in-depth exploration of this growing literature has become a relevant issue, both to identify the topical trends of COVID-related research and to zoom-in its sub-themes. This work proposes a novel methodology, called LDA2Net, which combines topic modelling and network analysis to investigate topics under their surface. Specifically, LDA2Net exploits the frequencies of pairs of consecutive words to reconstruct the network structure of topics discussed in the Cord-19 corpus. The results suggest that the effectiveness of topic models can be magnified by enriching them with word network representations, and by using the latter to display, analyse, and explore COVID-related topics at different levels of granularity.

==> LDA2Net Arxiv/table_topics.tex <==

% \begin{sidewaystable}
%   \centering
\centering
{\tiny

\begin{longtable}[ht]{c|l|l|l|l}
 
    % latex table generated in R 3.6.3 by xtable 1.8-4 package
% Wed Nov 10 13:29:43 2021
  \hline
Topic \# & Human label & 2-gram label & 3-gram label & 4-gram label \\ 
  \hline
   \hline
1 & protective devices & protection$\rightarrow$ equipment & protection$\rightarrow$ equipment$\rightarrow$ used & filtration$\rightarrow$ protection$\rightarrow$ equipment$\rightarrow$ used  \\ 
  2 & diagnostics & method$\rightarrow$ developed & method$\rightarrow$ developed$\rightarrow$ used & method$\rightarrow$ developed$\rightarrow$ rapid$\rightarrow$ sensitive  \\ 
  3 & statistical analysis (studies) & analysis$\rightarrow$ used & data$\rightarrow$ analysis$\rightarrow$ used & data$\rightarrow$ analysis$\rightarrow$ used$\rightarrow$ analyzed  \\ 
  4 & mortality rate related to infection & number$\rightarrow$ cases & number$\rightarrow$ cases$\rightarrow$ deaths & number$\rightarrow$ cases$\rightarrow$ deaths$\rightarrow$ per  \\ 
  5 & epidemic models & mathematical$\rightarrow$ model & epidemic$\rightarrow$ used$\rightarrow$ model & reproduction$\rightarrow$ number$\rightarrow$ R0$\rightarrow$ model  \\ 
  6 & retrospective clinical study & hospitalized$\rightarrow$ confirmed & hospitalized$\rightarrow$ confirmed$\rightarrow$ without & hospitalized$\rightarrow$ confirmed$\rightarrow$ without$\rightarrow$ diagnosed  \\ 
  7 & literature review & various$\rightarrow$ aspects & several$\rightarrow$ specific$\rightarrow$ aspects & aspects$\rightarrow$ human$\rightarrow$ papillomavirus$\rightarrow$ related  \\ 
  8 & clinical studies on illness development & mortality$\rightarrow$ rate & mortality$\rightarrow$ rate$\rightarrow$ patients & mortality$\rightarrow$ rate$\rightarrow$ patients$\rightarrow$ risk  \\ 
  9 & guidelines for clinical practice  management & clinical$\rightarrow$ practice & clinical$\rightarrow$ practice$\rightarrow$ management & clinical$\rightarrow$ practice$\rightarrow$ management$\rightarrow$ regarding  \\ 
  10 & statistical analysis  (scale assessment) & scale$\rightarrow$ scores & scale$\rightarrow$ scores$\rightarrow$ used & mean$\rightarrow$ score$\rightarrow$ scale$\rightarrow$ scores  \\ 
  11 & cellular immune response & inflammatory$\rightarrow$ macrophages & inflammatory$\rightarrow$ macrophages$\rightarrow$ including & inflammatory$\rightarrow$ loop$\rightarrow$ inflammation$\rightarrow$ production  \\ 
  12 & online education during pandemic & online$\rightarrow$ learning & online$\rightarrow$ learning$\rightarrow$ students & online$\rightarrow$ de$\rightarrow$ student$\rightarrow$ learning  \\ 
  13 & studies on origins & province$\rightarrow$ since & province$\rightarrow$ city$\rightarrow$ china & province$\rightarrow$ since$\rightarrow$ prevention$\rightarrow$ february  \\ 
  14 & public health response to pandemics & public$\rightarrow$ system & public$\rightarrow$ system$\rightarrow$ crisis & public$\rightarrow$ system$\rightarrow$ crisis$\rightarrow$ health  \\ 
  15 & reviews on recent therapeutical approaches & therapeutic$\rightarrow$ approaches & future$\rightarrow$ strategies$\rightarrow$ various & future$\rightarrow$ strategies$\rightarrow$ various$\rightarrow$ approaches  \\ 
  16 & mechanism of cell infection & ACE2$\rightarrow$ binding & ACE2$\rightarrow$ binding$\rightarrow$ expression & receptor$\rightarrow$ ACE2$\rightarrow$ binding$\rightarrow$ expression  \\ 
  17 &  ND & important$\rightarrow$ key & important$\rightarrow$ key$\rightarrow$ critical & important$\rightarrow$ key$\rightarrow$ critical$\rightarrow$ crucial  \\ 
  18 & study of variants & viral$\rightarrow$ genome & genome$\rightarrow$ sequences$\rightarrow$ identified & viral$\rightarrow$ genome$\rightarrow$ sequencing$\rightarrow$ sequence  \\ 
  19 & management of surgical procedures & surgical$\rightarrow$ procedures & surgical$\rightarrow$ procedures$\rightarrow$ patients & surgical$\rightarrow$ procedures$\rightarrow$ patients$\rightarrow$ procedure  \\ 
  20 & instrumental diagnosis & chest$\rightarrow$ CT & chest$\rightarrow$ CT$\rightarrow$ scan & chest$\rightarrow$ CT$\rightarrow$ scan$\rightarrow$ images  \\ 
  21 & contagion diffusion control & contact$\rightarrow$ tracing & contact$\rightarrow$ tracing$\rightarrow$ individuals & contact$\rightarrow$ tracing$\rightarrow$ persons$\rightarrow$ quarantine  \\ 
  22 & impact of pandemics on people (social relations) & social$\rightarrow$ distancing & social$\rightarrow$ distancing$\rightarrow$ isolation & social$\rightarrow$ distancing$\rightarrow$ isolation$\rightarrow$ support  \\ 
  23 & virus Cov-19 infection & virus$\rightarrow$ human & virus$\rightarrow$ human$\rightarrow$ viruses & SARS$\rightarrow$ MERS$\rightarrow$ virus$\rightarrow$ human  \\ 
  24 & pandemics history & help$\rightarrow$ us & help$\rightarrow$ us$\rightarrow$ make & help$\rightarrow$ us$\rightarrow$ make$\rightarrow$ one  \\ 
  25 & comparatiove  analysis of viremic levels & significantly$\rightarrow$ higher & levels$\rightarrow$ significantly$\rightarrow$ higher & significantly$\rightarrow$ higher$\rightarrow$ lower$\rightarrow$ level  \\ 
  26 & access to health of socio-economic groups & household$\rightarrow$ income & household$\rightarrow$ income$\rightarrow$ inequality & population$\rightarrow$ derived$\rightarrow$ nonprobability$\rightarrow$ sample  \\ 
  27 & Studies, evidences & evidence$\rightarrow$ suggest & evidence$\rightarrow$ suggest$\rightarrow$ studies & evidence$\rightarrow$ suggests$\rightarrow$ studies$\rightarrow$ needed  \\ 
  28 & methodological approaches & approach$\rightarrow$ problem & set$\rightarrow$ theory$\rightarrow$ method & approach$\rightarrow$ problem$\rightarrow$ time$\rightarrow$ algorithm  \\ 
  29 & ND & research$\rightarrow$ limitations & research$\rightarrow$ limitations$\rightarrow$ findings & research$\rightarrow$ limitations$\rightarrow$ development$\rightarrow$ process  \\ 
  30 & development in India & urban$\rightarrow$ population & urban$\rightarrow$ population$\rightarrow$ area & urban$\rightarrow$ population$\rightarrow$ planning$\rightarrow$ space  \\ 
  31 & digital technology & digital$\rightarrow$ version & digital$\rightarrow$ scanning$\rightarrow$ calorimetry & digital$\rightarrow$ scanning$\rightarrow$ calorimetry$\rightarrow$ technology  \\ 
  32 & Covid-19 literature & must$\rightarrow$ considered & one$\rightarrow$ especially$\rightarrow$ important & one$\rightarrow$ especially$\rightarrow$ important$\rightarrow$ reasons  \\ 
  33 & abstract structure & methods$\rightarrow$ results & methods$\rightarrow$ results$\rightarrow$ study & materials$\rightarrow$ methods$\rightarrow$ results$\rightarrow$ study  \\ 
  34 & prevention & prevention$\rightarrow$ measures & control$\rightarrow$ prevention$\rightarrow$ measures & prevention$\rightarrow$ measures$\rightarrow$ spread$\rightarrow$ strategies  \\ 
  35 & review studies & systematic$\rightarrow$ review & systematic$\rightarrow$ reviews$\rightarrow$ protocol & systematic$\rightarrow$ review$\rightarrow$ met$\rightarrow$ literature  \\ 
  36 & economic impact & tourism$\rightarrow$ development & tourism$\rightarrow$ development$\rightarrow$ business & tourism$\rightarrow$ development$\rightarrow$ business$\rightarrow$ market  \\ 
  37 & comparative studies & significantly$\rightarrow$ higher & significantly$\rightarrow$ higher$\rightarrow$ rate & significantly$\rightarrow$ higher$\rightarrow$ rate$\rightarrow$ compared  \\ 
  38 & effects of vitamin somministration & levels$\rightarrow$ supplementation & levels$\rightarrow$ supplementation$\rightarrow$ significantly & levels$\rightarrow$ supplementation$\rightarrow$ significantly$\rightarrow$ reduced  \\ 
  39 & data & data$\rightarrow$ collection & data$\rightarrow$ collection$\rightarrow$ analysis & data$\rightarrow$ collection$\rightarrow$ sources$\rightarrow$ used  \\ 
  40 & publication metadata & without$\rightarrow$ use & copyright$\rightarrow$ international$\rightarrow$ use & copyright$\rightarrow$ international$\rightarrow$ use$\rightarrow$ abstract  \\ 
  41 & impact on life quality \& sexual health & quality$\rightarrow$ life & quality$\rightarrow$ life$\rightarrow$ expectancy & quality$\rightarrow$ life$\rightarrow$ expectancy$\rightarrow$ health  \\ 
  42 & symptoms \& clinical manifestations & clinical$\rightarrow$ symptoms & gastrointestinal$\rightarrow$ infection$\rightarrow$ symptoms & clinical$\rightarrow$ symptoms$\rightarrow$ manifestations$\rightarrow$ reported  \\ 
  43 & effects of alcohool \& addictions & alcohol$\rightarrow$ medications & alcohol$\rightarrow$ medications$\rightarrow$ treatment & alcohol$\rightarrow$ medications$\rightarrow$ treatment$\rightarrow$ cannabis  \\ 
  44 & effects on patients with comorbidity & severe$\rightarrow$ disease & patients$\rightarrow$ severe$\rightarrow$ disease & patients$\rightarrow$ severe$\rightarrow$ disease$\rightarrow$ critical  \\ 
  45 & impact of air pollution & concentration$\rightarrow$ meteorological & concentration$\rightarrow$ meteorological$\rightarrow$ conditions & concentration$\rightarrow$ meteorological$\rightarrow$ conditions$\rightarrow$ observed  \\ 
  46 & correlation with heart disease & heart$\rightarrow$ failure & cardiac$\rightarrow$ arrest$\rightarrow$ patients & heart$\rightarrow$ failure$\rightarrow$ arrhythmias$\rightarrow$ acute  \\ 
  47 & ND & new$\rightarrow$ york & new$\rightarrow$ york$\rightarrow$ city & new$\rightarrow$ york$\rightarrow$ city$\rightarrow$ pandemic  \\ 
  48 & community & community$\rightarrow$ engagement & community$\rightarrow$ engagement$\rightarrow$ development & sustainable$\rightarrow$ strategies$\rightarrow$ partnerships$\rightarrow$ key  \\ 
  49 & stages & early$\rightarrow$ especially & early$\rightarrow$ especially$\rightarrow$ initial & early$\rightarrow$ especially$\rightarrow$ initial$\rightarrow$ results  \\ 
  50 & ND & higher$\rightarrow$ risk & adjusted$\rightarrow$ prevalence$\rightarrow$ ratio & adjusted$\rightarrow$ prevalence$\rightarrow$ ratio$\rightarrow$ among  \\ 
  51 & age and gender & older$\rightarrow$ people & older$\rightarrow$ people$\rightarrow$ individuals & older$\rightarrow$ people$\rightarrow$ individuals$\rightarrow$ higher  \\ 
  52 & interview studies & themes$\rightarrow$ emerged & themes$\rightarrow$ emerged$\rightarrow$ three & themes$\rightarrow$ emerged$\rightarrow$ three$\rightarrow$ key  \\ 
  53 & diagnostic tests efficacy & test$\rightarrow$ positive & test$\rightarrow$ positive$\rightarrow$ results & test$\rightarrow$ positive$\rightarrow$ results$\rightarrow$ tests  \\ 
  54 & french & de$\rightarrow$ patients & de$\rightarrow$ la$\rightarrow$ santé & de$\rightarrow$ la$\rightarrow$ santé$\rightarrow$ plus  \\ 
  55 & pandemic management & pandemic$\rightarrow$ response & pandemic$\rightarrow$ response$\rightarrow$ crisis & pandemic$\rightarrow$ response$\rightarrow$ crisis$\rightarrow$ management  \\ 
  56 & nursing programs residents & programs$\rightarrow$ program & programs$\rightarrow$ program$\rightarrow$ value & programs$\rightarrow$ program$\rightarrow$ value$\rightarrow$ virtual  \\ 
  57 & effective strategies & effective$\rightarrow$ strategies & effective$\rightarrow$ strategies$\rightarrow$ strategy & effective$\rightarrow$ strategies$\rightarrow$ strategy$\rightarrow$ approach  \\ 
  58 & policies for spread containment & control$\rightarrow$ measures & containment$\rightarrow$ interventions$\rightarrow$ implemented & containment$\rightarrow$ interventions$\rightarrow$ implemented$\rightarrow$ reduce  \\ 
  59 & technologies & surface$\rightarrow$ structure & process$\rightarrow$ storage$\rightarrow$ efficiency & process$\rightarrow$ storage$\rightarrow$ parameters$\rightarrow$ ph  \\ 
  60 & susceptibility to viral infection in epathitys & viral$\rightarrow$ infection & viral$\rightarrow$ infection$\rightarrow$ infections & viral$\rightarrow$ infection$\rightarrow$ infections$\rightarrow$ caused  \\ 
  61 & data for the study & analysis$\rightarrow$ used & data$\rightarrow$ analysis$\rightarrow$ used & data$\rightarrow$ analysis$\rightarrow$ used$\rightarrow$ study  \\ 
  62 & sociopolitical aspects & political$\rightarrow$ cultural & political$\rightarrow$ questions$\rightarrow$ social & ethical$\rightarrow$ issues$\rightarrow$ legal$\rightarrow$ political  \\ 
  63 & cancer therapy & cancer$\rightarrow$ treatment & cancer$\rightarrow$ treatment$\rightarrow$ patients & cancer$\rightarrow$ patients$\rightarrow$ diagnosis$\rightarrow$ therapy  \\ 
  64 & pediatry & children$\rightarrow$ adolescents & children$\rightarrow$ adolescents$\rightarrow$ young & children$\rightarrow$ adolescents$\rightarrow$ young$\rightarrow$ families  \\ 
  65 & oftalmic & ocular$\rightarrow$ surface & eye$\rightarrow$ ocular$\rightarrow$ surface & ocular$\rightarrow$ surface$\rightarrow$ conditions$\rightarrow$ presence  \\ 
  66 & comorbidity diabetes & chronic$\rightarrow$ diseases & chronic$\rightarrow$ diseases$\rightarrow$ disease & chronic$\rightarrow$ diseases$\rightarrow$ disease$\rightarrow$ diabetes  \\ 
  67 & rehabilitation after intervention & intervention$\rightarrow$ program & intervention$\rightarrow$ program$\rightarrow$ improve & intervention$\rightarrow$ program$\rightarrow$ improve$\rightarrow$ organizational  \\ 
  68 & pandemics in the us & state$\rightarrow$ local & state$\rightarrow$ local$\rightarrow$ federal & state$\rightarrow$ local$\rightarrow$ federal$\rightarrow$ level  \\ 
  69 & immunity \& specificity of response & igg$\rightarrow$ antibodies & igg$\rightarrow$ antibodies$\rightarrow$ antibody & igg$\rightarrow$ antibodies$\rightarrow$ antibody$\rightarrow$ response  \\ 
  70 & online (mis)information & information$\rightarrow$ sources & information$\rightarrow$ sources$\rightarrow$ related & information$\rightarrow$ sources$\rightarrow$ regarding$\rightarrow$ SDM  \\ 
  71 & variability & three$\rightarrow$ different & different$\rightarrow$ patterns$\rightarrow$ populations & three$\rightarrow$ different$\rightarrow$ patterns$\rightarrow$ populations  \\ 
  72 & healthcare & health$\rightarrow$ facilities & health$\rightarrow$ facilities$\rightarrow$ system & health$\rightarrow$ facilities$\rightarrow$ system$\rightarrow$ planning  \\ 
  73 & paper info & web$\rightarrow$ response & web$\rightarrow$ response$\rightarrow$ one & web$\rightarrow$ response$\rightarrow$ disclosure$\rightarrow$ including  \\ 
  74 & clinical cases reports & patient$\rightarrow$ presented & patient$\rightarrow$ presented$\rightarrow$ developed & patient$\rightarrow$ presented$\rightarrow$ developed$\rightarrow$ acute  \\ 
  75 & numbers & one$\rightarrow$ three & one$\rightarrow$ three$\rightarrow$ study & one$\rightarrow$ three$\rightarrow$ study$\rightarrow$ five  \\ 
  76 & UK pandemic timeline & first$\rightarrow$ time & first$\rightarrow$ time$\rightarrow$ UK & first$\rightarrow$ time$\rightarrow$ UK$\rightarrow$ weeks  \\ 
  77 & time \& duration & median$\rightarrow$ time & median$\rightarrow$ time$\rightarrow$ period & median$\rightarrow$ time$\rightarrow$ period$\rightarrow$ day  \\ 
  78 & geographic (countries) & world$\rightarrow$ health & around$\rightarrow$ world$\rightarrow$ health & around$\rightarrow$ world$\rightarrow$ health$\rightarrow$ response  \\ 
  79 & impact (on energy market) & paper$\rightarrow$ shows & paper$\rightarrow$ shows$\rightarrow$ impact & paper$\rightarrow$ shows$\rightarrow$ impact$\rightarrow$ examine  \\ 
  80 & antiviral treatments & antiviral$\rightarrow$ drugs & antiviral$\rightarrow$ drugs$\rightarrow$ used & antiviral$\rightarrow$ drugs$\rightarrow$ used$\rightarrow$ treatment  \\ 
  81 & medical organization and management & emergency$\rightarrow$ medicine & medical$\rightarrow$ personnel$\rightarrow$ emergency & emergency$\rightarrow$ medicine$\rightarrow$ doctors$\rightarrow$ management  \\ 
  82 & mental health & psychological$\rightarrow$ stress & stress$\rightarrow$ disorder$\rightarrow$ symptoms & psychological$\rightarrow$ stress$\rightarrow$ disorder$\rightarrow$ symptoms  \\ 
  83 & clinical studies on illness development & clinical$\rightarrow$ trial & clinical$\rightarrow$ trial$\rightarrow$ outcomes & clinical$\rightarrow$ trial$\rightarrow$ outcomes$\rightarrow$ registered  \\ 
  84 & questionnaire studies & study$\rightarrow$ participants & study$\rightarrow$ participants$\rightarrow$ conducted & study$\rightarrow$ participants$\rightarrow$ conducted$\rightarrow$ aimed  \\ 
  85 & damage mechansims & nervous$\rightarrow$ system & nervous$\rightarrow$ system$\rightarrow$ involvement & nervous$\rightarrow$ system$\rightarrow$ damage$\rightarrow$ including  \\ 
  86 & anti-inflammatory treatment & patients$\rightarrow$ received & patients$\rightarrow$ received$\rightarrow$ treatment & treatment$\rightarrow$ receiving$\rightarrow$ tocilizumab$\rightarrow$ systemic  \\ 
  87 & effects if pandemic & pandemic$\rightarrow$ impact & pandemic$\rightarrow$ impact$\rightarrow$ affected & pandemic$\rightarrow$ impact$\rightarrow$ affected$\rightarrow$ changes  \\ 
  88 & antiviral drug molecules & drug$\rightarrow$ target & antiviral$\rightarrow$ activity$\rightarrow$ compounds & antiviral$\rightarrow$ targets$\rightarrow$ identified$\rightarrow$ compounds  \\ 
  89 & risk factors & risk$\rightarrow$ factors & risk$\rightarrow$ factor$\rightarrow$ exposure & risk$\rightarrow$ factor$\rightarrow$ exposure$\rightarrow$ factors  \\ 
  90 & neurological and cognitive impairment & brain$\rightarrow$ including & neurologic$\rightarrow$ manifestations$\rightarrow$ including & neurologic$\rightarrow$ manifestations$\rightarrow$ including$\rightarrow$ brain  \\ 
  91 & respiratory failure & patients$\rightarrow$ severe & patients$\rightarrow$ severe$\rightarrow$ forms & patients$\rightarrow$ local$\rightarrow$ contestation$\rightarrow$ different  \\ 
  92 & predictive models & predictive$\rightarrow$ value & predictive$\rightarrow$ value$\rightarrow$ model & predictive$\rightarrow$ value$\rightarrow$ model$\rightarrow$ used  \\ 
  93 & behavioural studies & behavior$\rightarrow$ intention & positive$\rightarrow$ relationship$\rightarrow$ perceived & positive$\rightarrow$ relationship$\rightarrow$ perceived$\rightarrow$ behavioral  \\ 
  94 & sampling viral rna & viral$\rightarrow$ RNA & viral$\rightarrow$ RNA$\rightarrow$ load & viral$\rightarrow$ RNA$\rightarrow$ loads$\rightarrow$ samples  \\ 
  95 & pandemic impact & current$\rightarrow$ pandemic & current$\rightarrow$ pandemic$\rightarrow$ caused & current$\rightarrow$ pandemic$\rightarrow$ caused$\rightarrow$ coronavirus  \\ 
  96 & orthopedic traumas & wound$\rightarrow$ healing & wound$\rightarrow$ healing$\rightarrow$ repair & wound$\rightarrow$ healing$\rightarrow$ repair$\rightarrow$ attempt  \\ 
  97 & vaccine and immunity & vaccine$\rightarrow$ development & vaccine$\rightarrow$ development$\rightarrow$ efficacy & vaccine$\rightarrow$ development$\rightarrow$ candidate$\rightarrow$ vaccines  \\ 
  98 & icu and patinet care & ICU$\rightarrow$ patients & care$\rightarrow$ unit$\rightarrow$ patients & patients$\rightarrow$ admitted$\rightarrow$ hospitalized$\rightarrow$ hospital  \\ 
  99 & cellular mechanisms & gene$\rightarrow$ expression & gene$\rightarrow$ expression$\rightarrow$ genes & gene$\rightarrow$ expression$\rightarrow$ genes$\rightarrow$ involved  \\ 
  100 & pandemic & coronavirus$\rightarrow$ disease & novel$\rightarrow$ coronavirus$\rightarrow$ disease & coronavirus$\rightarrow$ disease$\rightarrow$ virus$\rightarrow$ spread  \\ 
  101 & health care personnel and pandemic & healthcare$\rightarrow$ workers & healthcare$\rightarrow$ workers$\rightarrow$ work & healthcare$\rightarrow$ workers$\rightarrow$ work$\rightarrow$ providers  \\ 
  102 & transplant & dental$\rightarrow$ treatment & clinical$\rightarrow$ course$\rightarrow$ dental & clinical$\rightarrow$ course$\rightarrow$ dental$\rightarrow$ treatment  \\ 
  103 & structural dynamics & complex$\rightarrow$ interactions & complex$\rightarrow$ interactions$\rightarrow$ structure & complex$\rightarrow$ interactions$\rightarrow$ structure$\rightarrow$ dynamics  \\ 
  104 & treatment of cardiovascular complications & stroke$\rightarrow$ acute & stroke$\rightarrow$ acute$\rightarrow$ severe & ischemic$\rightarrow$ thrombotic$\rightarrow$ outcomes$\rightarrow$ complications  \\ 
  105 & pandemic in selected countires & italy$\rightarrow$ spain & italy$\rightarrow$ spain$\rightarrow$ one & italy$\rightarrow$ spain$\rightarrow$ one$\rightarrow$ france  \\ 
  106 & spanish & de$\rightarrow$ la & de$\rightarrow$ la$\rightarrow$ pandemia & de$\rightarrow$ la$\rightarrow$ pandemia$\rightarrow$ esta  \\ 
  107 & AI models & deep$\rightarrow$ learning & deep$\rightarrow$ learning$\rightarrow$ de & deep$\rightarrow$ learning$\rightarrow$ de$\rightarrow$ performance  \\ 
  108 & physical activity and exercise & home$\rightarrow$ time & home$\rightarrow$ time$\rightarrow$ confinement & home$\rightarrow$ time$\rightarrow$ confinement$\rightarrow$ le  \\ 
  109 & statistics & control$\rightarrow$ groups & control$\rightarrow$ groups$\rightarrow$ significant & control$\rightarrow$ groups$\rightarrow$ significant$\rightarrow$ difference  \\ 
  110 & animal models \& in vitro & stem$\rightarrow$ reduced & stem$\rightarrow$ reduced$\rightarrow$ lung & stem$\rightarrow$ reduced$\rightarrow$ lung$\rightarrow$ human  \\ 
  111 & bacterial resistance to antibacterials & bacterial$\rightarrow$ infections & bacterial$\rightarrow$ infections$\rightarrow$ isolated & bacterial$\rightarrow$ pathogens$\rightarrow$ identified$\rightarrow$ found  \\ 
  112 & time studies & total$\rightarrow$ number & significant$\rightarrow$ increase$\rightarrow$ number & ED$\rightarrow$ emergency$\rightarrow$ visits$\rightarrow$ total  \\ 
  113 & body weight and metabolism & healthy$\rightarrow$ eating & BMI$\rightarrow$ obesity$\rightarrow$ metabolic & overweight$\rightarrow$ BMI$\rightarrow$ obesity$\rightarrow$ metabolic  \\ 
  114 & neo/perinatal infections & included$\rightarrow$ among & intrauterine$\rightarrow$ transplacental$\rightarrow$ flux & intrauterine$\rightarrow$ insemination$\rightarrow$ doses$\rightarrow$ low  \\ 
  115 & telemedicine & patient$\rightarrow$ care & telemedicine$\rightarrow$ visits$\rightarrow$ telehealth & telemedicine$\rightarrow$ visits$\rightarrow$ telehealth$\rightarrow$ access  \\ 
  116 & coronavirus disease progression & coronavirus$\rightarrow$ disease & coronavirus$\rightarrow$ disease$\rightarrow$ progression & coronavirus$\rightarrow$ de$\rightarrow$ un$\rightarrow$ autre  \\ 
  117 & report & reported$\rightarrow$ among & reported$\rightarrow$ among$\rightarrow$ less & reported$\rightarrow$ less$\rightarrow$ likely$\rightarrow$ report  \\ 
  118 & severe respiratory syndrome & acute$\rightarrow$ respiratory & acute$\rightarrow$ respiratory$\rightarrow$ syndrome & acute$\rightarrow$ respiratory$\rightarrow$ syndrome$\rightarrow$ coronavirus  \\ 
  119 & related works & related$\rightarrow$ pandemic & related$\rightarrow$ pandemic$\rightarrow$ including & status$\rightarrow$ related$\rightarrow$ pandemic$\rightarrow$ including  \\ 
  120 & research (publications) & scientific$\rightarrow$ research & scientific$\rightarrow$ studies$\rightarrow$ research & research$\rightarrow$ field$\rightarrow$ community$\rightarrow$ development  \\ 
   \hline
    \caption{Human labels and automated n-gram label proposals based on the proposed heuristic (see Section \ref{sec:methods}). Human labels have been defined by a medical expert by looking (only) to the list of the top 25 words of the topic.
    ND stands for not determined.
    }
    \label{tab:topic_labels}
\end{longtable}
}
   
    % \end{sidewaystable}


==> table_topics.tex <==

% \begin{sidewaystable}
%   \centering
\centering
{\tiny

\begin{longtable}[ht]{c|l|l|l|l}
 
    % latex table generated in R 3.6.3 by xtable 1.8-4 package
% Wed Nov 10 13:29:43 2021
  \hline
Topic \# & Human label & 2-gram label & 3-gram label & 4-gram label \\ 
  \hline
   \hline
1 & protective devices & protection$\rightarrow$ equipment & protection$\rightarrow$ equipment$\rightarrow$ used & filtration$\rightarrow$ protection$\rightarrow$ equipment$\rightarrow$ used  \\ 
  2 & diagnostics & method$\rightarrow$ developed & method$\rightarrow$ developed$\rightarrow$ used & method$\rightarrow$ developed$\rightarrow$ rapid$\rightarrow$ sensitive  \\ 
  3 & statistical analysis (studies) & analysis$\rightarrow$ used & data$\rightarrow$ analysis$\rightarrow$ used & data$\rightarrow$ analysis$\rightarrow$ used$\rightarrow$ analyzed  \\ 
  4 & mortality rate related to infection & number$\rightarrow$ cases & number$\rightarrow$ cases$\rightarrow$ deaths & number$\rightarrow$ cases$\rightarrow$ deaths$\rightarrow$ per  \\ 
  5 & epidemic models & mathematical$\rightarrow$ model & epidemic$\rightarrow$ used$\rightarrow$ model & reproduction$\rightarrow$ number$\rightarrow$ R0$\rightarrow$ model  \\ 
  6 & retrospective clinical study & hospitalized$\rightarrow$ confirmed & hospitalized$\rightarrow$ confirmed$\rightarrow$ without & hospitalized$\rightarrow$ confirmed$\rightarrow$ without$\rightarrow$ diagnosed  \\ 
  7 & literature review & various$\rightarrow$ aspects & several$\rightarrow$ specific$\rightarrow$ aspects & aspects$\rightarrow$ human$\rightarrow$ papillomavirus$\rightarrow$ related  \\ 
  8 & clinical studies on illness development & mortality$\rightarrow$ rate & mortality$\rightarrow$ rate$\rightarrow$ patients & mortality$\rightarrow$ rate$\rightarrow$ patients$\rightarrow$ risk  \\ 
  9 & guidelines for clinical practice  management & clinical$\rightarrow$ practice & clinical$\rightarrow$ practice$\rightarrow$ management & clinical$\rightarrow$ practice$\rightarrow$ management$\rightarrow$ regarding  \\ 
  10 & statistical analysis  (scale assessment) & scale$\rightarrow$ scores & scale$\rightarrow$ scores$\rightarrow$ used & mean$\rightarrow$ score$\rightarrow$ scale$\rightarrow$ scores  \\ 
  11 & cellular immune response & inflammatory$\rightarrow$ macrophages & inflammatory$\rightarrow$ macrophages$\rightarrow$ including & inflammatory$\rightarrow$ loop$\rightarrow$ inflammation$\rightarrow$ production  \\ 
  12 & online education during pandemic & online$\rightarrow$ learning & online$\rightarrow$ learning$\rightarrow$ students & online$\rightarrow$ de$\rightarrow$ student$\rightarrow$ learning  \\ 
  13 & studies on origins & province$\rightarrow$ since & province$\rightarrow$ city$\rightarrow$ china & province$\rightarrow$ since$\rightarrow$ prevention$\rightarrow$ february  \\ 
  14 & public health response to pandemics & public$\rightarrow$ system & public$\rightarrow$ system$\rightarrow$ crisis & public$\rightarrow$ system$\rightarrow$ crisis$\rightarrow$ health  \\ 
  15 & reviews on recent therapeutical approaches & therapeutic$\rightarrow$ approaches & future$\rightarrow$ strategies$\rightarrow$ various & future$\rightarrow$ strategies$\rightarrow$ various$\rightarrow$ approaches  \\ 
  16 & mechanism of cell infection & ACE2$\rightarrow$ binding & ACE2$\rightarrow$ binding$\rightarrow$ expression & receptor$\rightarrow$ ACE2$\rightarrow$ binding$\rightarrow$ expression  \\ 
  17 &  ND & important$\rightarrow$ key & important$\rightarrow$ key$\rightarrow$ critical & important$\rightarrow$ key$\rightarrow$ critical$\rightarrow$ crucial  \\ 
  18 & study of variants & viral$\rightarrow$ genome & genome$\rightarrow$ sequences$\rightarrow$ identified & viral$\rightarrow$ genome$\rightarrow$ sequencing$\rightarrow$ sequence  \\ 
  19 & management of surgical procedures & surgical$\rightarrow$ procedures & surgical$\rightarrow$ procedures$\rightarrow$ patients & surgical$\rightarrow$ procedures$\rightarrow$ patients$\rightarrow$ procedure  \\ 
  20 & instrumental diagnosis & chest$\rightarrow$ CT & chest$\rightarrow$ CT$\rightarrow$ scan & chest$\rightarrow$ CT$\rightarrow$ scan$\rightarrow$ images  \\ 
  21 & contagion diffusion control & contact$\rightarrow$ tracing & contact$\rightarrow$ tracing$\rightarrow$ individuals & contact$\rightarrow$ tracing$\rightarrow$ persons$\rightarrow$ quarantine  \\ 
  22 & impact of pandemics on people (social relations) & social$\rightarrow$ distancing & social$\rightarrow$ distancing$\rightarrow$ isolation & social$\rightarrow$ distancing$\rightarrow$ isolation$\rightarrow$ support  \\ 
  23 & virus Cov-19 infection & virus$\rightarrow$ human & virus$\rightarrow$ human$\rightarrow$ viruses & SARS$\rightarrow$ MERS$\rightarrow$ virus$\rightarrow$ human  \\ 
  24 & pandemics history & help$\rightarrow$ us & help$\rightarrow$ us$\rightarrow$ make & help$\rightarrow$ us$\rightarrow$ make$\rightarrow$ one  \\ 
  25 & comparatiove  analysis of viremic levels & significantly$\rightarrow$ higher & levels$\rightarrow$ significantly$\rightarrow$ higher & significantly$\rightarrow$ higher$\rightarrow$ lower$\rightarrow$ level  \\ 
  26 & access to health of socio-economic groups & household$\rightarrow$ income & household$\rightarrow$ income$\rightarrow$ inequality & population$\rightarrow$ derived$\rightarrow$ nonprobability$\rightarrow$ sample  \\ 
  27 & Studies, evidences & evidence$\rightarrow$ suggest & evidence$\rightarrow$ suggest$\rightarrow$ studies & evidence$\rightarrow$ suggests$\rightarrow$ studies$\rightarrow$ needed  \\ 
  28 & methodological approaches & approach$\rightarrow$ problem & set$\rightarrow$ theory$\rightarrow$ method & approach$\rightarrow$ problem$\rightarrow$ time$\rightarrow$ algorithm  \\ 
  29 & ND & research$\rightarrow$ limitations & research$\rightarrow$ limitations$\rightarrow$ findings & research$\rightarrow$ limitations$\rightarrow$ development$\rightarrow$ process  \\ 
  30 & development in India & urban$\rightarrow$ population & urban$\rightarrow$ population$\rightarrow$ area & urban$\rightarrow$ population$\rightarrow$ planning$\rightarrow$ space  \\ 
  31 & digital technology & digital$\rightarrow$ version & digital$\rightarrow$ scanning$\rightarrow$ calorimetry & digital$\rightarrow$ scanning$\rightarrow$ calorimetry$\rightarrow$ technology  \\ 
  32 & Covid-19 literature & must$\rightarrow$ considered & one$\rightarrow$ especially$\rightarrow$ important & one$\rightarrow$ especially$\rightarrow$ important$\rightarrow$ reasons  \\ 
  33 & abstract structure & methods$\rightarrow$ results & methods$\rightarrow$ results$\rightarrow$ study & materials$\rightarrow$ methods$\rightarrow$ results$\rightarrow$ study  \\ 
  34 & prevention & prevention$\rightarrow$ measures & control$\rightarrow$ prevention$\rightarrow$ measures & prevention$\rightarrow$ measures$\rightarrow$ spread$\rightarrow$ strategies  \\ 
  35 & review studies & systematic$\rightarrow$ review & systematic$\rightarrow$ reviews$\rightarrow$ protocol & systematic$\rightarrow$ review$\rightarrow$ met$\rightarrow$ literature  \\ 
  36 & economic impact & tourism$\rightarrow$ development & tourism$\rightarrow$ development$\rightarrow$ business & tourism$\rightarrow$ development$\rightarrow$ business$\rightarrow$ market  \\ 
  37 & comparative studies & significantly$\rightarrow$ higher & significantly$\rightarrow$ higher$\rightarrow$ rate & significantly$\rightarrow$ higher$\rightarrow$ rate$\rightarrow$ compared  \\ 
  38 & effects of vitamin somministration & levels$\rightarrow$ supplementation & levels$\rightarrow$ supplementation$\rightarrow$ significantly & levels$\rightarrow$ supplementation$\rightarrow$ significantly$\rightarrow$ reduced  \\ 
  39 & data & data$\rightarrow$ collection & data$\rightarrow$ collection$\rightarrow$ analysis & data$\rightarrow$ collection$\rightarrow$ sources$\rightarrow$ used  \\ 
  40 & publication metadata & without$\rightarrow$ use & copyright$\rightarrow$ international$\rightarrow$ use & copyright$\rightarrow$ international$\rightarrow$ use$\rightarrow$ abstract  \\ 
  41 & impact on life quality \& sexual health & quality$\rightarrow$ life & quality$\rightarrow$ life$\rightarrow$ expectancy & quality$\rightarrow$ life$\rightarrow$ expectancy$\rightarrow$ health  \\ 
  42 & symptoms \& clinical manifestations & clinical$\rightarrow$ symptoms & gastrointestinal$\rightarrow$ infection$\rightarrow$ symptoms & clinical$\rightarrow$ symptoms$\rightarrow$ manifestations$\rightarrow$ reported  \\ 
  43 & effects of alcohool \& addictions & alcohol$\rightarrow$ medications & alcohol$\rightarrow$ medications$\rightarrow$ treatment & alcohol$\rightarrow$ medications$\rightarrow$ treatment$\rightarrow$ cannabis  \\ 
  44 & effects on patients with comorbidity & severe$\rightarrow$ disease & patients$\rightarrow$ severe$\rightarrow$ disease & patients$\rightarrow$ severe$\rightarrow$ disease$\rightarrow$ critical  \\ 
  45 & impact of air pollution & concentration$\rightarrow$ meteorological & concentration$\rightarrow$ meteorological$\rightarrow$ conditions & concentration$\rightarrow$ meteorological$\rightarrow$ conditions$\rightarrow$ observed  \\ 
  46 & correlation with heart disease & heart$\rightarrow$ failure & cardiac$\rightarrow$ arrest$\rightarrow$ patients & heart$\rightarrow$ failure$\rightarrow$ arrhythmias$\rightarrow$ acute  \\ 
  47 & ND & new$\rightarrow$ york & new$\rightarrow$ york$\rightarrow$ city & new$\rightarrow$ york$\rightarrow$ city$\rightarrow$ pandemic  \\ 
  48 & community & community$\rightarrow$ engagement & community$\rightarrow$ engagement$\rightarrow$ development & sustainable$\rightarrow$ strategies$\rightarrow$ partnerships$\rightarrow$ key  \\ 
  49 & stages & early$\rightarrow$ especially & early$\rightarrow$ especially$\rightarrow$ initial & early$\rightarrow$ especially$\rightarrow$ initial$\rightarrow$ results  \\ 
  50 & ND & higher$\rightarrow$ risk & adjusted$\rightarrow$ prevalence$\rightarrow$ ratio & adjusted$\rightarrow$ prevalence$\rightarrow$ ratio$\rightarrow$ among  \\ 
  51 & age and gender & older$\rightarrow$ people & older$\rightarrow$ people$\rightarrow$ individuals & older$\rightarrow$ people$\rightarrow$ individuals$\rightarrow$ higher  \\ 
  52 & interview studies & themes$\rightarrow$ emerged & themes$\rightarrow$ emerged$\rightarrow$ three & themes$\rightarrow$ emerged$\rightarrow$ three$\rightarrow$ key  \\ 
  53 & diagnostic tests efficacy & test$\rightarrow$ positive & test$\rightarrow$ positive$\rightarrow$ results & test$\rightarrow$ positive$\rightarrow$ results$\rightarrow$ tests  \\ 
  54 & french & de$\rightarrow$ patients & de$\rightarrow$ la$\rightarrow$ santé & de$\rightarrow$ la$\rightarrow$ santé$\rightarrow$ plus  \\ 
  55 & pandemic management & pandemic$\rightarrow$ response & pandemic$\rightarrow$ response$\rightarrow$ crisis & pandemic$\rightarrow$ response$\rightarrow$ crisis$\rightarrow$ management  \\ 
  56 & nursing programs residents & programs$\rightarrow$ program & programs$\rightarrow$ program$\rightarrow$ value & programs$\rightarrow$ program$\rightarrow$ value$\rightarrow$ virtual  \\ 
  57 & effective strategies & effective$\rightarrow$ strategies & effective$\rightarrow$ strategies$\rightarrow$ strategy & effective$\rightarrow$ strategies$\rightarrow$ strategy$\rightarrow$ approach  \\ 
  58 & policies for spread containment & control$\rightarrow$ measures & containment$\rightarrow$ interventions$\rightarrow$ implemented & containment$\rightarrow$ interventions$\rightarrow$ implemented$\rightarrow$ reduce  \\ 
  59 & technologies & surface$\rightarrow$ structure & process$\rightarrow$ storage$\rightarrow$ efficiency & process$\rightarrow$ storage$\rightarrow$ parameters$\rightarrow$ ph  \\ 
  60 & susceptibility to viral infection in epathitys & viral$\rightarrow$ infection & viral$\rightarrow$ infection$\rightarrow$ infections & viral$\rightarrow$ infection$\rightarrow$ infections$\rightarrow$ caused  \\ 
  61 & data for the study & analysis$\rightarrow$ used & data$\rightarrow$ analysis$\rightarrow$ used & data$\rightarrow$ analysis$\rightarrow$ used$\rightarrow$ study  \\ 
  62 & sociopolitical aspects & political$\rightarrow$ cultural & political$\rightarrow$ questions$\rightarrow$ social & ethical$\rightarrow$ issues$\rightarrow$ legal$\rightarrow$ political  \\ 
  63 & cancer therapy & cancer$\rightarrow$ treatment & cancer$\rightarrow$ treatment$\rightarrow$ patients & cancer$\rightarrow$ patients$\rightarrow$ diagnosis$\rightarrow$ therapy  \\ 
  64 & pediatry & children$\rightarrow$ adolescents & children$\rightarrow$ adolescents$\rightarrow$ young & children$\rightarrow$ adolescents$\rightarrow$ young$\rightarrow$ families  \\ 
  65 & oftalmic & ocular$\rightarrow$ surface & eye$\rightarrow$ ocular$\rightarrow$ surface & ocular$\rightarrow$ surface$\rightarrow$ conditions$\rightarrow$ presence  \\ 
  66 & comorbidity diabetes & chronic$\rightarrow$ diseases & chronic$\rightarrow$ diseases$\rightarrow$ disease & chronic$\rightarrow$ diseases$\rightarrow$ disease$\rightarrow$ diabetes  \\ 
  67 & rehabilitation after intervention & intervention$\rightarrow$ program & intervention$\rightarrow$ program$\rightarrow$ improve & intervention$\rightarrow$ program$\rightarrow$ improve$\rightarrow$ organizational  \\ 
  68 & pandemics in the us & state$\rightarrow$ local & state$\rightarrow$ local$\rightarrow$ federal & state$\rightarrow$ local$\rightarrow$ federal$\rightarrow$ level  \\ 
  69 & immunity \& specificity of response & igg$\rightarrow$ antibodies & igg$\rightarrow$ antibodies$\rightarrow$ antibody & igg$\rightarrow$ antibodies$\rightarrow$ antibody$\rightarrow$ response  \\ 
  70 & online (mis)information & information$\rightarrow$ sources & information$\rightarrow$ sources$\rightarrow$ related & information$\rightarrow$ sources$\rightarrow$ regarding$\rightarrow$ SDM  \\ 
  71 & variability & three$\rightarrow$ different & different$\rightarrow$ patterns$\rightarrow$ populations & three$\rightarrow$ different$\rightarrow$ patterns$\rightarrow$ populations  \\ 
  72 & healthcare & health$\rightarrow$ facilities & health$\rightarrow$ facilities$\rightarrow$ system & health$\rightarrow$ facilities$\rightarrow$ system$\rightarrow$ planning  \\ 
  73 & paper info & web$\rightarrow$ response & web$\rightarrow$ response$\rightarrow$ one & web$\rightarrow$ response$\rightarrow$ disclosure$\rightarrow$ including  \\ 
  74 & clinical cases reports & patient$\rightarrow$ presented & patient$\rightarrow$ presented$\rightarrow$ developed & patient$\rightarrow$ presented$\rightarrow$ developed$\rightarrow$ acute  \\ 
  75 & numbers & one$\rightarrow$ three & one$\rightarrow$ three$\rightarrow$ study & one$\rightarrow$ three$\rightarrow$ study$\rightarrow$ five  \\ 
  76 & UK pandemic timeline & first$\rightarrow$ time & first$\rightarrow$ time$\rightarrow$ UK & first$\rightarrow$ time$\rightarrow$ UK$\rightarrow$ weeks  \\ 
  77 & time \& duration & median$\rightarrow$ time & median$\rightarrow$ time$\rightarrow$ period & median$\rightarrow$ time$\rightarrow$ period$\rightarrow$ day  \\ 
  78 & geographic (countries) & world$\rightarrow$ health & around$\rightarrow$ world$\rightarrow$ health & around$\rightarrow$ world$\rightarrow$ health$\rightarrow$ response  \\ 
  79 & impact (on energy market) & paper$\rightarrow$ shows & paper$\rightarrow$ shows$\rightarrow$ impact & paper$\rightarrow$ shows$\rightarrow$ impact$\rightarrow$ examine  \\ 
  80 & antiviral treatments & antiviral$\rightarrow$ drugs & antiviral$\rightarrow$ drugs$\rightarrow$ used & antiviral$\rightarrow$ drugs$\rightarrow$ used$\rightarrow$ treatment  \\ 
  81 & medical organization and management & emergency$\rightarrow$ medicine & medical$\rightarrow$ personnel$\rightarrow$ emergency & emergency$\rightarrow$ medicine$\rightarrow$ doctors$\rightarrow$ management  \\ 
  82 & mental health & psychological$\rightarrow$ stress & stress$\rightarrow$ disorder$\rightarrow$ symptoms & psychological$\rightarrow$ stress$\rightarrow$ disorder$\rightarrow$ symptoms  \\ 
  83 & clinical studies on illness development & clinical$\rightarrow$ trial & clinical$\rightarrow$ trial$\rightarrow$ outcomes & clinical$\rightarrow$ trial$\rightarrow$ outcomes$\rightarrow$ registered  \\ 
  84 & questionnaire studies & study$\rightarrow$ participants & study$\rightarrow$ participants$\rightarrow$ conducted & study$\rightarrow$ participants$\rightarrow$ conducted$\rightarrow$ aimed  \\ 
  85 & damage mechansims & nervous$\rightarrow$ system & nervous$\rightarrow$ system$\rightarrow$ involvement & nervous$\rightarrow$ system$\rightarrow$ damage$\rightarrow$ including  \\ 
  86 & anti-inflammatory treatment & patients$\rightarrow$ received & patients$\rightarrow$ received$\rightarrow$ treatment & treatment$\rightarrow$ receiving$\rightarrow$ tocilizumab$\rightarrow$ systemic  \\ 
  87 & effects if pandemic & pandemic$\rightarrow$ impact & pandemic$\rightarrow$ impact$\rightarrow$ affected & pandemic$\rightarrow$ impact$\rightarrow$ affected$\rightarrow$ changes  \\ 
  88 & antiviral drug molecules & drug$\rightarrow$ target & antiviral$\rightarrow$ activity$\rightarrow$ compounds & antiviral$\rightarrow$ targets$\rightarrow$ identified$\rightarrow$ compounds  \\ 
  89 & risk factors & risk$\rightarrow$ factors & risk$\rightarrow$ factor$\rightarrow$ exposure & risk$\rightarrow$ factor$\rightarrow$ exposure$\rightarrow$ factors  \\ 
  90 & neurological and cognitive impairment & brain$\rightarrow$ including & neurologic$\rightarrow$ manifestations$\rightarrow$ including & neurologic$\rightarrow$ manifestations$\rightarrow$ including$\rightarrow$ brain  \\ 
  91 & respiratory failure & patients$\rightarrow$ severe & patients$\rightarrow$ severe$\rightarrow$ forms & patients$\rightarrow$ local$\rightarrow$ contestation$\rightarrow$ different  \\ 
  92 & predictive models & predictive$\rightarrow$ value & predictive$\rightarrow$ value$\rightarrow$ model & predictive$\rightarrow$ value$\rightarrow$ model$\rightarrow$ used  \\ 
  93 & behavioural studies & behavior$\rightarrow$ intention & positive$\rightarrow$ relationship$\rightarrow$ perceived & positive$\rightarrow$ relationship$\rightarrow$ perceived$\rightarrow$ behavioral  \\ 
  94 & sampling viral rna & viral$\rightarrow$ RNA & viral$\rightarrow$ RNA$\rightarrow$ load & viral$\rightarrow$ RNA$\rightarrow$ loads$\rightarrow$ samples  \\ 
  95 & pandemic impact & current$\rightarrow$ pandemic & current$\rightarrow$ pandemic$\rightarrow$ caused & current$\rightarrow$ pandemic$\rightarrow$ caused$\rightarrow$ coronavirus  \\ 
  96 & orthopedic traumas & wound$\rightarrow$ healing & wound$\rightarrow$ healing$\rightarrow$ repair & wound$\rightarrow$ healing$\rightarrow$ repair$\rightarrow$ attempt  \\ 
  97 & vaccine and immunity & vaccine$\rightarrow$ development & vaccine$\rightarrow$ development$\rightarrow$ efficacy & vaccine$\rightarrow$ development$\rightarrow$ candidate$\rightarrow$ vaccines  \\ 
  98 & icu and patinet care & ICU$\rightarrow$ patients & care$\rightarrow$ unit$\rightarrow$ patients & patients$\rightarrow$ admitted$\rightarrow$ hospitalized$\rightarrow$ hospital  \\ 
  99 & cellular mechanisms & gene$\rightarrow$ expression & gene$\rightarrow$ expression$\rightarrow$ genes & gene$\rightarrow$ expression$\rightarrow$ genes$\rightarrow$ involved  \\ 
  100 & pandemic & coronavirus$\rightarrow$ disease & novel$\rightarrow$ coronavirus$\rightarrow$ disease & coronavirus$\rightarrow$ disease$\rightarrow$ virus$\rightarrow$ spread  \\ 
  101 & health care personnel and pandemic & healthcare$\rightarrow$ workers & healthcare$\rightarrow$ workers$\rightarrow$ work & healthcare$\rightarrow$ workers$\rightarrow$ work$\rightarrow$ providers  \\ 
  102 & transplant & dental$\rightarrow$ treatment & clinical$\rightarrow$ course$\rightarrow$ dental & clinical$\rightarrow$ course$\rightarrow$ dental$\rightarrow$ treatment  \\ 
  103 & structural dynamics & complex$\rightarrow$ interactions & complex$\rightarrow$ interactions$\rightarrow$ structure & complex$\rightarrow$ interactions$\rightarrow$ structure$\rightarrow$ dynamics  \\ 
  104 & treatment of cardiovascular complications & stroke$\rightarrow$ acute & stroke$\rightarrow$ acute$\rightarrow$ severe & ischemic$\rightarrow$ thrombotic$\rightarrow$ outcomes$\rightarrow$ complications  \\ 
  105 & pandemic in selected countires & italy$\rightarrow$ spain & italy$\rightarrow$ spain$\rightarrow$ one & italy$\rightarrow$ spain$\rightarrow$ one$\rightarrow$ france  \\ 
  106 & spanish & de$\rightarrow$ la & de$\rightarrow$ la$\rightarrow$ pandemia & de$\rightarrow$ la$\rightarrow$ pandemia$\rightarrow$ esta  \\ 
  107 & AI models & deep$\rightarrow$ learning & deep$\rightarrow$ learning$\rightarrow$ de & deep$\rightarrow$ learning$\rightarrow$ de$\rightarrow$ performance  \\ 
  108 & physical activity and exercise & home$\rightarrow$ time & home$\rightarrow$ time$\rightarrow$ confinement & home$\rightarrow$ time$\rightarrow$ confinement$\rightarrow$ le  \\ 
  109 & statistics & control$\rightarrow$ groups & control$\rightarrow$ groups$\rightarrow$ significant & control$\rightarrow$ groups$\rightarrow$ significant$\rightarrow$ difference  \\ 
  110 & animal models \& in vitro & stem$\rightarrow$ reduced & stem$\rightarrow$ reduced$\rightarrow$ lung & stem$\rightarrow$ reduced$\rightarrow$ lung$\rightarrow$ human  \\ 
  111 & bacterial resistance to antibacterials & bacterial$\rightarrow$ infections & bacterial$\rightarrow$ infections$\rightarrow$ isolated & bacterial$\rightarrow$ pathogens$\rightarrow$ identified$\rightarrow$ found  \\ 
  112 & time studies & total$\rightarrow$ number & significant$\rightarrow$ increase$\rightarrow$ number & ED$\rightarrow$ emergency$\rightarrow$ visits$\rightarrow$ total  \\ 
  113 & body weight and metabolism & healthy$\rightarrow$ eating & BMI$\rightarrow$ obesity$\rightarrow$ metabolic & overweight$\rightarrow$ BMI$\rightarrow$ obesity$\rightarrow$ metabolic  \\ 
  114 & neo/perinatal infections & included$\rightarrow$ among & intrauterine$\rightarrow$ transplacental$\rightarrow$ flux & intrauterine$\rightarrow$ insemination$\rightarrow$ doses$\rightarrow$ low  \\ 
  115 & telemedicine & patient$\rightarrow$ care & telemedicine$\rightarrow$ visits$\rightarrow$ telehealth & telemedicine$\rightarrow$ visits$\rightarrow$ telehealth$\rightarrow$ access  \\ 
  116 & coronavirus disease progression & coronavirus$\rightarrow$ disease & coronavirus$\rightarrow$ disease$\rightarrow$ progression & coronavirus$\rightarrow$ de$\rightarrow$ un$\rightarrow$ autre  \\ 
  117 & report & reported$\rightarrow$ among & reported$\rightarrow$ among$\rightarrow$ less & reported$\rightarrow$ less$\rightarrow$ likely$\rightarrow$ report  \\ 
  118 & severe respiratory syndrome & acute$\rightarrow$ respiratory & acute$\rightarrow$ respiratory$\rightarrow$ syndrome & acute$\rightarrow$ respiratory$\rightarrow$ syndrome$\rightarrow$ coronavirus  \\ 
  119 & related works & related$\rightarrow$ pandemic & related$\rightarrow$ pandemic$\rightarrow$ including & status$\rightarrow$ related$\rightarrow$ pandemic$\rightarrow$ including  \\ 
  120 & research (publications) & scientific$\rightarrow$ research & scientific$\rightarrow$ studies$\rightarrow$ research & research$\rightarrow$ field$\rightarrow$ community$\rightarrow$ development  \\ 
   \hline
    \caption{Human labels and automated n-gram label proposals based on the proposed heuristic (see Section \ref{sec:methods}). Human labels have been defined by a medical expert by looking (only) to the list of the top 25 words of the topic.
    ND stands for not determined.
    }
    \label{tab:topic_labels}
\end{longtable}
}
   
    % \end{sidewaystable}

